Reward Selection with Noisy Observations

We study a fundamental problem in optimization under uncertainty. There are $n$ boxes; each box $i$ contains a hidden reward $x_i$. Rewards are drawn i.i.d. from an unknown distribution $\mathcal{D}$. For each box $i$, we see $y_i$, an unbiased estimate of its reward, which is drawn from a Normal distribution with known standard deviation $\sigma_i$ (and an unknown mean $x_i$). Our task is to select a single box, with the goal of maximizing our reward. This problem captures a wide range of applications, e.g. ad auctions, where the hidden reward is the click-through rate of an ad. Previous work in this model [BKMR12] proves that the naive policy, which selects the box with the largest estimate $y_i$, is suboptimal, and suggests a linear policy, which selects the box $i$ with the largest $y_i - c \cdot \sigma_i$, for some $c > 0$. However, no formal guarantees are given about the performance of either policy (e.g., whether their expected reward is within some factor of the optimal policy's reward). In this work, we prove that both the naive policy and the linear policy are arbitrarily bad compared to the optimal policy, even when $\mathcal{D}$ is well-behaved, e.g. has monotone hazard rate (MHR), and even under a "small tail" condition, which requires that not too many boxes have arbitrarily large noise. On the flip side, we propose a simple threshold policy that gives a constant approximation to the reward of a prophet (who knows the realized values $x_1, \dots, x_n$) under the same "small tail" condition. We prove that when this condition is not satisfied, even an optimal clairvoyant policy (that knows $\mathcal{D}$) cannot get a constant approximation to the prophet, even for MHR distributions, implying that our threshold policy is optimal against the prophet benchmark, up to constants.

==> discussion.tex <==
\section{Discussion}

While we have structurally defined both the small noise and large noise regimes and showed both positive and negative results for each, the current definitions permit weird cases where some ``easier'' $\std$ is in the large noise regime, while other ``harder'' $\std$ are in the small noise regime. For example, take $c = 0.1$, and consider these two following initializations of $\std$'s:
\begin{itemize}
    \item $\std_1 = \left\{\underbrace{0, 0, \dots, 0}_{\text{$n^c - 1$ copies}}, \underbrace{\frac{\E[\D_{n:n}]}{18c \sqrt{2 \ln n}} + \epsilon, \frac{\E[\D_{n:n}]}{18c \sqrt{2 \ln n}} + \epsilon, \dots, \frac{\E[\D_{n:n}]}{18c \sqrt{2 \ln n}} + \epsilon}_{\text{$n - n^c + 1$ copies}}\right\}$ for any $\epsilon > 0$.
    \item $\std_2 = \left\{\underbrace{\frac{\E[\D_{n:n}]}{18 \sqrt{2c \ln n}}, \frac{\E[\D_{n:n}]}{18 \sqrt{2c \ln n}}, \dots, \frac{\E[\D_{n:n}]}{18c \sqrt{2c \ln n}}}_{\text{$n^c$ copies}}, \underbrace{\infty, \infty, \dots, \infty}_{\text{$n - n^c$ copies}}\right\}$.
\end{itemize}

Under our definitions, $\std_1 \in \badMHR{\D}{n,c}$ while $\std_2 \in \goodMHR{\D}{n,c}$. However, purely from visual inspection, it is obvious $\std_1$ is much easier for any algorithm to deal with than $\std_2$, as even a simple algorithm such as ``only picking the best box out of boxes that have $0$ noise'' can win a constant approximation in this case. Therefore, it is an open question of how we can analyze the performance of the optimal algorithm on any $\std$ \emph{instance-wise}, and whether there is any simple-yet-powerful algorithm that takes the advantage of the actual values of $\std$ (recall that both $\IgnoreLarge$ and $\IgnoreLargeExp$ do not look at the values of $\std$ after the initial sorting phase).

% \subsection{Technical highlights}

% At a high level, the downfall of both $\Naive$ and $\Linear$ algorithms is that they treat very different types of boxes in a virtually identical manner: $\Naive$ does not take in the noise information at all, while $\Linear$ utilizes this information in a very crude way, and discount boxes with massively different order of noises with the same weight.
% Intuitively, a good algorithm should ``spot'' large noise boxes and ignore them, and both $\Naive$ and $\Linear$ do not perform a good job at spotting large noise boxes.

% However, large noises are relative to $\D$, which the algorithm does not have any information on other than the noisy samples $y_i$. We circumvent this problem by essentially ``randomly'' deciding the cutoff between the small noise and the large noise boxes (which is manifested in the design of $\IgnoreLarge$ and $\IgnoreLargeExp$), with the idea being that if there are many small noise boxes, then random cutoff has a good chance of selecting a non-trivial amount of small noise boxes. This idea turns out to work as \Cref{thm:ignore-large} and \Cref{thm:ignore-large-expo-mhr} suggest. Furthermore, when there are not many small noise boxes, we also expect that no algorithms can perform well, which is formalized in \Cref{thm:opt-bad-vs-prophet} and \Cref{thm: opt bad vs random}.
